5G Network on Wings: A Deep Reinforcement Learning Approach to the UAV-based Integrated Access and Backhaul

Fast and reliable wireless communication has become a critical demand in human life. In the case of mission-critical (MC) scenarios, for instance, when natural disasters strike, providing ubiquitous connectivity becomes challenging by using traditional wireless networks. In this context, unmanned aerial vehicle (UAV) based aerial networks offer a promising alternative for fast, flexible, and reliable wireless communications. Due to unique characteristics such as mobility, flexible deployment, and rapid reconfiguration, drones can readily change location dynamically to provide on-demand communications to users on the ground in emergency scenarios. As a result, the usage of UAV base stations (UAV-BSs) has been considered an appropriate approach for providing rapid connection in MC scenarios. In this paper, we study how to control multiple UAV-BSs in both static and dynamic environments. We use a system-level simulator to model an MC scenario in which a macro BS of a cellular network is out of service and multiple UAV-BSs are deployed using integrated access and backhaul (IAB) technology to provide coverage for users in the disaster area. With the data collected from the system-level simulation, a deep reinforcement learning algorithm is developed to jointly optimize the three-dimensional placement of these multiple UAV-BSs, which adapt their 3-D locations to the on-ground user movement. The evaluation results show that the proposed algorithm can support the autonomous navigation of the UAV-BSs to meet the MC service requirements in terms of user throughput and drop rate.

==> sections/biography.tex <==
\begin{IEEEbiographynophoto}{First A. Author} (M'76--SM'81--F'87) and the other authors may 
include biographies at the end of regular papers. Biographies are often not 
included in conference-related papers. This author became a Member (M) of 
IEEE in 1976, a Senior Member (SM) in 1981, and a Fellow (F) in 1987.
\end{IEEEbiographynophoto}

==> sections/signaling_procedure.tex <==
\section{Functional Framework for RAN Intelligence}
In this section, we introduce a functional framework for enabling an intelligent radio access network (RAN). 
\begin{comment}
We also propose several signaling procedures based on this functional framework to apply ML to the considered use case described in the previous section.
\end{comment}
%\subsection{Functional Framework for RAN Intelligence}
%3GPP standardization status: Refer to 3GPP standards
%Introduce our proposed framework: Module by module
To provide guidance on designing intelligent RAN enabled by ML, the 3rd Generation Partnership Project (3GPP) initiated a study on enhancement for data collection for 5G NR in Release 17 \cite{3gpp.37.817}, where high-level principles and corresponding functional framework for RAN intelligence are introduced. This functional framework consists of different ML functionalities, including Data Collection, Model Training, Model Inference, and Actor. Based on this functional framework, we define each ML functionality for our considered use case as follows. 

The Data Collection function is responsible for collecting input data (e.g., measurements and performance metrics from interested users and the related BSs) for ML. The collected data is divided into two sub-sets as training data and inference data. They are provided to the Model Training and Model Inference functions, respectively. The Data Collection function may also receive feedback from other learning functions and adjust its configuration (e.g., data collection periodicity and collected data type) accordingly.

The Model Training function performs the ML model training, validation, and testing of the ML model using the training data. Then, it sends the ML model to the Model Inference function. 

The Model Inference function provides the learning outcome using the ML model received from the Model Training function and the inference data delivered from the Data Collection function. 

The Actor function receives the output from the Model Inference function and triggers or performs corresponding actions, e.g., navigating the UAV-BS to a new position in the considered use case.

To enable the RAN intelligence during implementation, the Model Training and Model Inference functions can be mounted on the intelligent nodes (e.g. UAV-BS or donor-BS in this paper) to analyse collected data and generate ML-related model parameters. It is preferred to deploy these functions close to the data source to reduce the overhead caused by transferring data. However, it is not mandatory to deploy Model Training and Model Inference at the same node. To reduce the power consumption and data transferring during the model training procedure, the node can be only deployed with the Model Inference function and performance intelligent action based on the model generated from the Model Training function of the other intelligent nodes. The data exchange between the intelligent nodes can be enabled by the existing RAN interfaces.

\begin{comment}
%Introduce reward function if needed
\begin{figure}[]
\centering
\subfigure[Case 1: UAV-BS Hosting ML Model]{
\begin{minipage}[b]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures/SignalingProcedureCase1.png} 

%\label{Tilt-5PercTput}
\end{minipage}
}
\subfigure[Case 2: Donor-BS Hosting ML Model]{
\begin{minipage}[b]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures/SignalingProcedureCase2.png}

%\label{Tilt-50PercTput}
\end{minipage}
}
\subfigure[Case 3: UAV-BS Hosting ML Model \& Donor-BS as Central Server]{
\begin{minipage}[b]{0.45\textwidth}
\includegraphics[width=\textwidth]{figures/SignalingProcedureCase3.png}

%\label{Tilt-DropRate}
\end{minipage}
}
\vspace{-5pt}
\caption{Signaling procedures to support applying ML for the considered use case}

\label{fig:SignalingProcedure}
\end{figure}


\subsection{Intelligence-Based Signaling Procedure}
In this subsection, we present three different signaling procedures to illustrate how the proposed functional framework can be utilized to support applying centralized or distributed ML for the considered use case, i.e., the 3-D location of a UAV-BS in an IAB network architecture. Depending on where the ML model is hosted and how the ML algorithm is executed (distributed or centralized), three major scenarios are introduced in the following subsections. Here, we consider a single-hop IAB operation. The UAV-BS is connected to its donor-BS via a direct single-hop wireless backhaul link, and it provides wireless access links to connected users. In addition, we assume that the data collection for ML is triggered by the donor-BS. The proposed signaling procedures can also be extended to other cases like multi-hop IAB operations and UAV-BS triggered data collection. 



%Case 1
\subsubsection{Case 1: UAV-BS Hosting ML Model}
For Case 1, as shown in Figure \ref{fig:SignalingProcedure}(a), the UAV-BS is connected to a donor-BS via single-hop wireless backhauling, and it will provide wireless access links to MC UEs within its coverage. Data collection for optimizing the UAV-BS's configuration and deployment is triggered by a donor-BS, while the collected data can be raw data based on the measurements, key performance indicators (KPIs), or post-processed data. The ML related functions, including Data Collection, Model Training, Model Inference, and Actor, are all hosted in the UAV-BS, which reduces the signaling overhead and latency caused by ML-related information exchange between the UAV-BS and the other network entities. If multiple UAV-BSs are used in the considered single-hop IAB operation scenario, the proposed singling procedure in Case 1 allows each UAV-BS to make its local decision independently. Hence, this signaling procedure can be used to support distributed ML, and it consists of the following key steps:

\begin{enumerate}[1):]

\item Data requests triggered by a donor-BS: After a UAV-BS completes its network integration procedure, or when a UAV-BS mobility event has been detected (e.g., a UAV-BS has adjusted its location), the donor-BS triggers data collection to assist the UAV-BS in optimizing its configuration and deployment by sending a data request message to the relevant users and BSs. 

\item Data collection at the UAV-BS: After receiving the data request, MC users, the donor-BS, and related BSs on the ground will send the requested data to the UAV-BS. The collected data can include: a) data collected by the UAV-BS itself, e.g., from its connected MC users, radio measurements, and onboard sensors; b) data firstly reported from a set of users and a set of BSs on the ground, and then forwarded to the UAV-BS. 

\item Learning process in the UAV-BS: After processing the collected data, the Model Training and Model Inference functions at the UAV-BS are initiated accordingly. When the model training procedure is finished, a set of ML-related parameters are generated corresponding to the trained model. Then, the Model Inference function will develop the suggested deployment strategy and configuration based on the trained model and collected inference data. 

\item The UAV-BS takes action: Based on the output of the Model Inference, the Actor function in the UAV-BS performs location position adjustment and other suggested configurations.

\item The UAV-BS sends feedback to its donor-BS, who can then forward the feedback or action recommendations to the other related BSs.

\item With the feedback from the UAV-BS as input data, the donor-BS and/or the related BSs adjust their configuration (e.g., antenna tilt, transmit power, etc.). Finally, the donor-BS stops requesting data.
\end{enumerate}

In the above procedure, steps 2)-6) can repeat till certain criteria are fulfilled (e.g., the ML algorithm can steadily provide optimized output). The donor-BS can then stop the learning process by sending a stop data reporting message to its connected users and the other related BSs.

%Case 2
\subsubsection{Case 2: Donor-BS Hosting ML Model}
For Case 2, as shown in Figure \ref{fig:SignalingProcedure}(b), the major difference from Case 1 is that all ML-related functions are hosted at the donor-BS. This can relax the hardware requirements and reduce the computational complexity for the UAV-BS, which can in turn reduce the power consumption and increase the flying time of the UAV-BS. The signaling procedure can be used to support centralized ML algorithms and it consists of the following key steps:

\noindent 1)-3): Similar to Case 1, except that the data collection and learning process are performed at the donor-BS.

\begin{enumerate}[1):]\setcounter{enumi}{3}

\item The donor-BS sends feedback to the UAV-BSs and other related BSs. The feedback includes recommendations on the configuration/adjustment of these BSs.

\item The UAV-BS takes action: The UAV-BS performs (re)configuration and/or movement based on the feedback from the Actor function in its donor-BS.

\item With the feedback from the donor-BS as input data, the related BSs adjust their configuration (e.g., antenna tilt, transmit power). Finally, the donor-BS stops requesting data.
\end{enumerate}

Similar to case 1, step 2)-6) in Case 2 can also repeat till certain criteria are fulfilled (e.g., the ML algorithm can steadily provide optimized output).

%Case 3
\subsubsection{Case 3: UAV-BS Hosting ML Model \& Donor-BS as Central Server}
For Case 3, as shown in Figure \ref{fig:SignalingProcedure}(c), a signaling procedure is proposed to support hybrid ML algorithms, where a centralized ML model is maintained at a central service (i.e., the donor-BS in our case) and a local copy of the ML model is distributed to each UAV-BS. The donor-BS aggregates the training results received from the UAV-BSs and updates its central ML model. After the UAV-BS finishes its model training, a refined local ML model will be generated and feedback to the donor. The signaling procedure consists of the following key steps:

\begin{enumerate}[1):]

\item Model update triggered by a donor-BS: After a UAV-BS completes its network integration procedure, or when a UAV-BS mobility event has been detected (e.g., a UAV-BS has adjusted its location), the donor-BS triggers the central ML model updates by sending a copy of the centralized ML model to the UAV-BS. 

\item Data collection at the UAV-BS: After receiving the global learning model, the UAV-BS triggers data collection to optimize its configuration and deployment by sending a data request message to the relevant users and its donor-BS. The collected data can be the same as the candidate parameters in Case 1. 

\item Learning process in the UAV-BS: Each UAV BS can gradually learn and update the received global model based on its locally collected data. When the model update is finished, a refined local model is generated and will be sent back to its donor-BS. 

\item The UAV-BS takes action: Based on the output of the local ML Model Inference, the Actor function in the UAV-BS performs location adjustment and other suggested configurations.

\item The UAV-BS sends feedback to the central server (donor-BS). The feedback includes training results (e.g., trained local model) from the UAV-BS.

\item Based on the feedback from the UAV-BS, the donor-BS aggregates the training results (e.g., trained local model) transferred from all related UAV BSs, and updates the centralized ML model. 

\item Repeat the above process if needed.

\end{enumerate}

\end{comment}

%Future consideration


\begin{comment}
%Table
\begin{table}[h]
\caption{Summary for three ML-based signaling cases}
\label{Table:SigCase}
\setlength{\tabcolsep}{3pt}

\begin{tabular}{|m{75pt}<{\centering}|m{75pt}<{\centering}|m{75pt}<{\centering}|}
\hline
Case Index& 
%Backhaul Link Type& 
%Trigger for Data Collection&
\makecell[c]{AI/ML Model\\Hosting Node}&
AI/ML Type\\
\hline
Case 1& 
%Single-hop& 
UAV-BS&
Distributed \\
Case 2& 
%Single-hop& 
Donor-BS&
Centralized \\
Case 3& 
%Single-hop& 
UAV-BS&
Hybrid \\
\hline
\end{tabular}
\end{table}
\end{comment}




